Energy Efficient Data Recovery from Corrupted LoRa Frames

High frame-corruption is widely observed in Long Range Wide Area Networks (LoRaWAN) due to the coexistence with other networks in ISM bands and an Aloha-like MAC layer. LoRa's Forward Error Correction (FEC) mechanism is often insufficient to retrieve corrupted data. In fact, real-life measurements show that at least one-fourth of received transmissions are corrupted. When more frames are dropped, LoRa nodes usually switch over to higher spreading factors (SF), thus increasing transmission times and increasing the required energy. This paper introduces ReDCoS, a novel coding technique at the application layer that improves recovery of corrupted LoRa frames, thus reducing the overall transmission time and energy invested by LoRa nodes by several-fold. ReDCoS utilizes lightweight coding techniques to pre-encode the transmitted data. Therefore, the inbuilt Cyclic Redundancy Check (CRC) that follows is computed based on an already encoded data. At the receiver, we use both the CRC and the coded data to recover data from a corrupted frame beyond the built-in Error Correcting Code (ECC). We compare the performance of ReDCoS to (I) the standard FEC of vanilla-LoRaWAN, and to (ii) RS coding applied as ECC to the data of LoRaWAN. The results indicated a 54x and 13.5x improvement of decoding ratio, respectively, when 20 data symbols were sent. Furthermore, we evaluated ReDCoS on-field using LoRa SX1261 transceivers showing that it outperformed RS-coding by factor of at least 2x (and up to 6x) in terms of the decoding ratio while consuming 38.5% less energy per correctly received transmission.

==> sections/large.tex <==
\subsection{Decoding time of large payloads}
Although the main focus of this work is applications with small payloads, transmissions of relatively larger payloads --for example of $50$ symbols-- can occur.
However, the encoding is very lightweight but the decoding of larger payloads could be problematic.
%Sherlock's encoder is quite lightweight and suitable for resource limited devices. 
%However, the Sherlock's decoder is a bit more complicated. 
Let us take an example.  

\begin{example}
Assuming that a payload with $k = 20$, $t = 4$, $l = 4$, and $SER = 0.1$ needs $0.14$ \,s to decode, we focus on finding the time needed for a payload with $k = 40$, $t = 8$, $l = 4$, and $SER = 0.1$. 
The number of $k$-combinations increases by a factor of $\frac{C(48,40)}{C(24,20)} = 35,512$.
Further, using Gaussian elimination, the complexity increases by $\frac{40^3}{20^3}=8$.
Thus, the total complexity increases with a factor of $284,096$ and hence the expected decoding time would be $284,096 \times 0.14 \approx 39,773.44~s \approx 11~hours$.
\end{example}

\begin{figure}[t]
\center
\includegraphics[width=0.49\textwidth]{pic/idea-long.pdf}
\caption{Solving the problem for large payloads (a) Making groups of symbols, (b) Proposed idea for large symbols.}
\label{long}
\end{figure}

\begin{figure}[t]
\center
\includegraphics[width=0.49\textwidth]{pic/idea-long-ex.pdf}
\caption{ An example of the proposed idea for large payloads.}
\label{long-ex}
\end{figure}

\textbf{Solution.} In this section, we provide the solution for the aforementioned problem that leads to immense decoding times. 
A possible approach is to consider each part of $k+t$ symbols as one group with $Q$ symbols, as shown in Fig.~\ref{long}.~(a), both at the encoder and the decoder. 
Then, every error correcting group is a linear combination of the grouped parts of payload. 
This decreases the computational complexity dramatically as the number of combinations and Gaussian elimination complexity for a payload with $k, t$, and $Q$ parameters are equal to the ones for $k^\prime = \frac{k}{Q}$ and $t^\prime = \frac{t}{Q}$ without making groups of symbols. 
However, the above decreases drastically the decoding probability as even one corrupted symbol renders its whole corresponding group useless. Then, any combination made by the decoder using that group leads to corrupted results. 
%if one symbol is corrupted in a given group, any combination made by the decoder using that group is corrupted, too.
This worsens by increasing $Q$ for larger payloads, as it increases the probability of at least one corrupted symbol per group. 

Therefore, as shown in Fig.~\ref{long}.~(b), although we still define groups of symbols, we take advantage of the fact that the $i$-th symbol in a given group is only dependent to the $i$-th symbol in other groups. 
This relationship is shown in Fig.~\ref{long}.~(b) with red lines.
The formal decoding algorithm for a given received frame with large payload is detailed in
algorithm\ref{alg:decoder2}, where $K=\frac{k}{Q}$ and $T =\frac{t}{Q}$ denote the number of groups in the payload and the number of groups in the extra error correcting symbols.

\begin{algorithm}[t]
	\footnotesize
	\DontPrintSemicolon
	\caption{ReDCoS' decoder for large payloads:}
	\KwInput{received payload $pay\_rec$, received error correcting symbols $ecs\_rec$, received CRC $CRC\_rec$, minimum\_num\_CRC\_symbol\_matches $H$}
    \KwOutput{healthy payload $pay\_hth$}
    $CRC\_table \leftarrow [\{\} \times Q]$ \tcp*{list of pairs of (CRC:\#repetition)}
    $can\_parts[[] \times Q]$ \tcp*{list of lists of candidate parts}
	\texttt{Step 1:} Check if the received encoded payload is healthy.\;
	$i \leftarrow find\_CRC(pay\_rec, ecs\_rec)$\;
	\If{$i == CRC\_rec$}{ 
	    $return(pay\_hth = pay\_rec)$ \tcp*{End: SUCCESS}
	}
	\For{$j = \{1,2,...,C(K+T,K)\}$}{
	    \texttt{Step 2:} Generate a healthy encoded payload candidate: Try a $K$-combination\;
	    $y \leftarrow \{\}.size(k+t)$\;
	    $y \leftarrow select\_K\_groups(pay\_rec,ecs\_rec)$\;
	    $y \leftarrow calculate\_left\_T\_groups(y)$\;
	    $i \leftarrow find\_CRC(y)$\;
	    \texttt{Step 3:} Check if the candidate matches the received CRC\;
	    \If{$i == CRC\_rec$}{ 
	    $pay\_hth = pick\_first\_k\_symbols(y)$\; 
	    $return(pay\_hth)$ \tcp*{End: SUCCESS}
	    }
	    \texttt{Step 4:} calculate $Q$ CRCs where $CRC_m$ is for the $m$-th symbols of groups.\;
	    $parts \leftarrow slice\_to\_Q\_parts(y)$ \tcp*{$part_m$ includes the $m$-th symbol of groups.}
	    \For{$m = \{0,1,...,Q-1\}$}{
	    $i \leftarrow find\_CRC(part_m)$\;
	    \If{$!find\_key(i,CRC\_table[m])$}{
	    $CRC\_table[m][i] = 1$\;
	    }
	    \Else{
	    $CRC\_table[m][i] += 1$\;
	    \texttt{Step 5:} Majority voting.\;
	    \If{$CRC\_table[m][i] == K+1$}{
	    \texttt{Step 6: Save/check this part}
	    $can\_parts[m].append(part_m)$\;
	    \If{$check\_min\_one\_candidate\_per\_list(can\_parts)$}{\texttt{Step 4:} Try all combinations of combining parts.\;
	    $y2 \leftarrow generate\_one\_mixture()$\;
	    $i \leftarrow find\_CRC(y2)$\;
	    $x \leftarrow find\_\#similar\_symbols(i,CRC\_rec)$\;
	    \texttt{Step 6:} Verify the recovered CRC.\;
	    \If{$x \geq H$}{
	    $pay\_hth = pick\_first\_k\_symbols(y)$\;
	    $return(pay\_hth)$ \tcp*{End: SUCCESS}
	    }
	    }
	    }
	    }
	    }
	    
	}
	\texttt{Step 7:} return failed decoding\;
	$return("Failed\; Decoding")$  \tcp*{End: Failed}\;
	
	\label{alg:decoder2}
\end{algorithm}









































 
% %Decoding is very similar to the scheme described in Sec.~\ref{sub:idea}.
% To decode the data, $K$ groups are chosen out of $K+T$ groups. 
% The remained $T$ groups are constructed using the selected $K$ groups. 
% The receiver calculates a CRC for the current symbols. The receiver checks whether the calculated CRC is equal to the received CRC.
% If so, the selected groups are healthy and the payload is retrieved (\textbf{SUCCESS}). 
% If not, the receiver calculates $Q$ CRCs, where, CRC$_i$ is calculated for the $i$-th symbol per group.
% The receiver tracks these CRCs, checking whether each CRC$_i$ has been seen previously for each $i$-th symbol per group in order to find the best candidates for the $i$-th symbols in the groups, separately. 
% If CRC$_i$ have not been spotted for the $i$-th symbols previously, the receiver saves this CRC for the $i$-th symbols and assigns a counter equal to $1$ to it, as in the single-symbol case discussed previously.
% If the CRC is seen previously, the receiver increases the associated counter. 
% Then, it checks if the counter is equal to $K+1$. 
% If so, ????????????????????????????????????????? you should now describe what if it matches or not. 
% After checking all the $i$-th CRCs for the current combination, the receiver continue the process with another combination.
% Decoding fails if the receiver checks all the combinations and does not find the correct CRC.
% Let us elaborate this technique using an example.
\begin{example}
Fig.~\ref{long-ex} shows an example where $Q=2$. $x_1$ and $r_2$ are corrupted during the transmission. 
The payload has four groups. 
Thus, for each combination, the receiver selects four groups and tries to generate the rest of the groups.
In the combination \#1, the groups number $1,3,4$ ,and $7$ are chosen. 
This means that $x^*_1$ is one of the selected symbols. 
Since, it is the first symbol in the group, all the first symbols in the generated groups are corrupted. 
But, the second generated symbols in each group are healthy.
Accordingly, in combination \#$1$, all the second symbols in the groups are healthy. 
Using the same reasoning, in combination \#$2$, all the first symbols of the groups are healthy. 
By putting these two healthy parts together, healthy payload can be retrieved. 
\end{example}
Note that in this paper, we assume $Q=1$ unless otherwise stated which corresponds to not making groups of symbols. 


==> sections/later.tex <==
\section{introduction}
Numerous heterogeneous applications in Smart Cities and the Industry 4.0 operate using the data provided by IoT-devices that monitor the ambient environment. 
These smart devices are usually energy constrained and require single hop transmissions over large distances for their data-packets. 
To address the above need, the advances in RF-technology led to the rise of Low Power Wide Area Networks (LPWAN), providing energy efficient and multi-kilometer communication to IoT-devices. 
\begin{figure}[t]
\center
\includegraphics[width=0.5\textwidth]{pic/lora.pdf}
\caption{A typical LoRaWAN network}
\label{lora}
\end{figure} 

%\subsection{LoRa and LoRaWAN}
Long Range WAN (LoRaWAN)~\cite{sornin2015lorawan} is a popular LPWAN technology which --compared to others (e.g., NB-IoT, SigFox)-- offers a "plug \& play" approach, providing an easily accessible network to both corporate and private parties. 
LoRa networks use sub-GHz license-free ISM bands, allowing their deployment without costs for spectrum usage. 
LoRaWAN enables inexpensive, secure, and power-efficient communication for energy restricted IoT-devices that transmit packets of small payloads over large time intervals. 
Fig.~\ref{lora} shows a typical LoRaWAN network consisting of end-devices, gateways, a network server, and an application server. 

The physical layer of LoRaWAN is based on LoRa and is proprietary, owned by Semtech. 
LoRa is a frequency modulation technique derived from Chirp Spread Spectrum~(CSS) mechanism. 
This modulation technique gives LoRa-signals increased robustness against noise, enabling long range data transmissions of several kilometers even with low transmission power, as signals get detected even below the noise-level~\cite{Juha,Liando}. 
A LoRaWAN network operates under a star of stars topology. As observed in Fig.~\ref{lora}, the data transmitted by the end-devices can be received by one or more gateways. 
The gateways forward the data --using the Internet-- to the network server which is responsible for removing the duplicate messages and forwarding them to the application server. LoRaWAN is an open-standard by the LoRa-Alliance~\cite{LoRaAlliance}. 
LoRa networks offer a wide range of configurable transmission parameters --Spreading Factor (SF), transmission power, carrier frequency, channel bandwidth, forward error correction, and coding rate~($CR$)-- in order to connect high numbers of devices~\cite{Bor2017lora}. 
LoRa encodes each symbol, $s$, by $N = 2^{SF}$ \textit{chips} 
%where $SF$ is the \textit{spreading factor} 
and $SF \in {7, 8, ..., 12}$.
Accordingly, a symbol $s$ is of length $SF$ bits and $s \in \mathcal{S}$ where $\mathcal{S} = {0, 1, ..., N-1}$. 
Low $SF$s have high data rates --reaching up to 50\,kbps-- and relatively shorter transmission times but support shorter transmission ranges. 
For thorough information regarding LoRa and LoRaWAN, refer to the official sources~\cite{Semtech,LoRaAlliance}. 

\subsection{Packet Corruption in LoRaWAN}
However, LoRa transmissions often suffer from corruption either to multiple symbols or to bursts of symbols. This renders LoRa-packets useless, and happens due to the following: 
\begin{itemize}
    \item LoRa-packets can reach gateways located multiple kilometers away; around 5\,km in urban and 15\,km in rural scenarios\cite{CentenaroReview}. Over such long distances the corrupting effect of multipath propagation and physical phenomena, like shadowing and scattering, is predominant. In Non-Line of Sight (NLoS) conditions urban clutter intensifies the above phenomena. 
    \item By operating in ISM bands LoRaWAN shares spectrum with other contending networks which interfere to LoRa-packets, and their transmissions corrupt LoRa-symbols. 
    \item The Medium Access Control (MAC) layer of LoRaWAN is unslotted and Aloha-like, wherein every device transmits its packet upon generation without sensing the channel for any ongoing transmission. This aggravates further the issue of corrupted packets as it increases collisions. 
\end{itemize} 
Since most IoT-applications involve data-driven systems of sensors and actuators, the minimization of data-corruption is critical for their seamless operation. 
Further, data-loss leads to increased energy consumption due to packet retransmisssions, so the recovery of LoRa-transmissions is crucial to sustain the battery-life of the already constrained LoRa-devices. 

For data recovery, LoRa-modems use Forward Error Correction (FEC), and specifically Hamming codes\cite{elshabrawy2019evaluation}, allowing $CR$ of $\frac{4}{4+x}$ where $x \in \{1,2,3,4\}$. Namely, every $4$~bit part of the packet is encoded into $4+x$ bits. 
$CR$-values of 4/5 and 4/6 are capable only of error detection, while 4/7 and 4/8 can correct single errors or detect double errors. 
Uplink messages transmitted by end-devices can use $4$-bit Cyclic Redundancy Check (CRC) for their headers and $16$-bit CRC at the end of their payloads for error detection. 
Moreover, the payload itself ends with $32$-bit Message Integrity Code~(MIC), i.e., a Cipher-based Message Authentication Code~(CMAC) that assigns a specific signature to every end-device.
%calculated with a device-specific key shared between the end-device and the network server.checks the message integrity and 

\subsection{Constraints}
As observed through real-case experiments performed by Rahmadhani and Kuipers, Marcelis \textit{et al.}, and Bor \textit{et al.}, the correction capability of the simple FEC mechanism of LoRa gets outperformed by the sheer numbers of corrupted symbols, which often lead to failed CRC-checks and dropped payloads. 
Rahmadhani and Kuipers showed up to 32\% of transmissions being corrupted in experiments wherein gateways were positioned 0.5-21.5\,km away of multiple end-devices\cite{Rahmadhani}. 
Marcelis \textit{et al.} observed up to 53\% packet-loss due to corruption as LoRa-devices moved at 6\,km from the nearest gateway\cite{Marcelis}. 
Bor \textit{et al.} observed even up to 100\% corrupted packet reception ratio at the gateway when a LoRa-transmission was interfered by another LoRa-transmission under specific delay-offsets\cite{bor2016lora}.
Additionally, we performed real-case experiments using LoRaWAN modules to investigate the level of corruption in LoRa-transmissions. Out of the 5000 packets transmitted per case, we found 29\%-53\% being received with corrupted symbols. 
The experiments took place indoors in Line of Sight (LoS), using operation frequency of $868.1$~MHz, bandwidth of $125$~kHz, and SF8. 
%, and isotropic antennas with $0$~dBi gain. The propagation was based on the log-distance model, with direct Line of Sight between the transmitter and receiver. 
Table.~\ref{ta:rec} depicts the portion of healthy and corrupted received packets for our experiments. 

\begin{table}[bt!]
\begin{center}
\begin{threeparttable}[b]
	\footnotesize
	\caption{Packet Reception Measurement}
	\vspace*{-5mm}
	\label{ta:rec}
	\begin{tabular}{|c|c|c|}
		\hline
		payload size~[B]  & Healthy Received & Corrupted Received\\
		\hline
	    $14$ & $35.24\%$ & $28.45\%$\\
		\hline
		$18$ & $45.28\%$ & $36.71\%$\\
		\hline
		$24$ & $16.54\%$ & $53.25\%$\\
		\hline
		$28$ & $23.93\%$ & $49.72\%$ \\
		\hline 
	\end{tabular}
\end{threeparttable}
\end{center}
\end{table}

%As the total number of IoT-devices is projected to 41 billion by 2027~\cite{bosch}, a large portion of such devices will be communicating through LoRaWAN or ISM-contending protocols. 
The aforementioned reports necessitate novel coding algorithms on the application layer of LoRaWAN. 
%in order to enable connectivity for the future highly pervasive IoT-applications of Smart Cities and Industry 4.0. 
However, the algorithms need to adhere to the constraints posed by LoRaWAN: 
\begin{itemize}
    \item Their application should not require any changes in the gateways and the existing infrastructure of LoRa networks. 
    \item They should not be based on feedback from the gateway as it increases the message overhead and the energy consumption due to extra listening times. 
    \item The introduced symbol redundancy due to encoding should be minimal, especially for high SFs, because the allowed payload size is limited (i.e., 51\,B for SF10-SF12). 
\end{itemize}

\subsection{Contributions}
To this point, we introduce ReDCoS, \underline{Re}covery of \underline{D}ata of \underline{Co}rrupted \underline{S}ignals; a novel coding scheme for the application layer of LoRa networks. ReDCoS operates proactively before the LoRa-FEC mechanism is applied. 
ReDCoS encodes the payload of a LoRa-packet independently, and adds a limited number of encoded symbols at the end of the payload. Thus, the following FEC mechanism of LoRa adds redundancy over an already encoded piece of information, boosting the error-correcting capability of the system. 
Nevertheless, ReDCoS can substitute completely the existing FEC mechanism of LoRaWAN. 

Our contributions are the following: 
\begin{enumerate}
    \item We design ReDCoS, a novel application layer coding technique that allows the recovery of LoRa transmissions well beyond built-in error correcting capability (see Sect.~\ref{system}). 
    \item We provide mathematical analysis of ReDCoS, finding the probability of successful decoding (see Sect.~\ref{analysis}). 
    \item We evaluate the performance of ReDCoS not only numerically but also experimentally, by conducting on-field experiments using LoRa-devices and a gateway.  We show that ReDCoS improves the decoding ratio up to a factor of 6.12, compared to using Reed-Solomon codes for error correction (see Sect.~\ref{evaluation}). 
\end{enumerate}
\textcolor{red}{NIKOS: Add paper-map if there's space left at the end.}
\section{Related Works}
Marcelis \textit{et al.} introduced DaRe, a coding scheme against data-loss, operating at the application layer of LoRaWAN. DaRe combines convolutional and fountain codes, providing 21\% higher data recovery than LoRaWAN's repetition coding\cite{Marcelis}. 
%, while reducing consumption due to transmissions of 10\,B-packets by 42\%. 
%Tkachenko \textit{et al.}\cite{Tkachenko} used a new ensemble of neural network tools to predict the missing IoT data. 
%In [12], the 
Coutaud and Tourancheau designed CCARR which uses Reed Solomon (RS) at the frame-level. CCARR transmits encoded super-frames, involving application data and redundancy data (RS-frames). 
%By dynamically adapting the size of RS-frames, 
CCARR guarantees high packet delivery ratio (even 100\%) over lossy channels\cite{Coutaud}. 
Borkotoky \textit{et al.} propose two application-layer coding schemes --windowed and selective coding-- for delay-intolerant LoRaWANs with minimum feedback. Windowed mechanism encodes by accounting all the non-delivered and non-expired transmitted symbols, while selective coding picks certain among them based on feedback\cite{Borkotoky}. 
%Selective coding outperforms all other schemes in terms of reducing delivery failure rate. 
Tsimbalo \textit{at al.} exploit the redundancy that CRC adds to the encoded data by applying iterative algorithms --ADMM and BP-- on the decoding side. They correct up to 35\% of corrupted BLE-packets without consuming any extra energy at the transmitter side\cite{Tsimbalo}. 
Sant'Ana \textit{et al.} combine two coding techniques of LPWANs: transmission of packet-replicas, RT, and transmission of encoded packets using linear operations like XORs, CT. Their hybrid coding scheme, which is optimized for LoRaWAN, can support the transmissions by more devices than RT and CT alone while extending their battery lifetime\cite{SantAna}. 
Chen \textit{et al.} extend the lifetime and communication range of LoRaWAN, by introducing eLoRa, which recovers the correct parts of a packet by applying Luby codes (LT) on several versions of the packet that are received by multiple gateways. Further, eLoRa optimizes physical layer parameters to best serve lifetime and range requirements\cite{Chen}. 
Coutaud \textit{et al.} characterize the behavior of LoRa-channels in urban scenarios and adapt the specifics of ADR's FEC and retransmission schemes, in order to improve the current Adaptive Data Rate (ADR) mechanism of LoRaAWAN. \cite{CoutaudADR}. 

Contrary to the previous works, ReDCoS does not require any change to the LoRa-standard (PHY). 
Further, ReDCoS does not need buffer and/or feedback downlinks for its operation, keeping message-overhead low. 
Finally, although it uses simple encoder --respecting the low computational capabilities of LoRa-devices-- it outperforms RS schemes. 


==> sections/pattern_study.tex <==
\section{The Pattern of the CRCs Repetitions}
%
As stated in Sec.~\ref{sub:idea}, using the proposed scheme, the receiver tries different combinations.
In total ${k+t \choose k}$ unique combinations exist.
The CRC for each combination might be different from the previous ones (considering the same received packet) or equal to one or more of them. 
In this subsection, we study the pattern of the CRCs repetitions.
Initially, we concentrate on the case where all different combinations are tried. 
Then, we will focus on the CRCs repetitions for a successful data retrieval and for a failed data retrieval.
For now, we consider using brute force for trying the different combinations.

\subsection{Trying all the Combinations}

\begin{lemma}
If two combinations generate the same CRC while this is not due to collisions in CRC calculation, then the associated CRC will be repeated ${k+b \choose k} $ times in case of trying all different combinations where $b$ is the number of symbols in each of them which are not available in the other one.
\end{lemma}

\begin{proof}
If two combinations generate the same CRC, it means they have generated the same encoded data as well. 
Every symbol in any combination will appear in the associated encoded data.
Each of the combinations has $b$ symbols which the other one does not have; However, these symbols are generated in the encoded datas as the datas are equal.
Accordingly, $k+b$ symbols exist which any $k$-combination out of them generate the same encoded data and hence the same CRC.
The number of $k$-combinations out of $k+b$ elements is equal to ${k+b \choose k}$.
Accordingly, the associated CRC will be repeated ${k+b \choose k}$ times.  
\end{proof}

\begin{figure}[t]
\center
\includegraphics[width=0.45\textwidth]{pic/proof.pdf}
\caption{An example for two combinations generating the same CRC. Any combination made out of the symbols of these two combinations generate the same CRC. 
The received symbols and generated symbols are shown with \textit{$\hat{}$} and $\bar{}$, respectively. a) received symbols, b) selected symbols and generated symbols, c) Any combination made from these symbols generate the same CRC.
Note that considering the equality of the two CRC, $\hat{x_2} = \bar{x_2}$ and $\hat{r_2} = \bar{r_2}$.}
\label{proof}
\end{figure} 

Fig.~\ref{proof} shows an example where two combinations generate the same encoded data. The received symbols and the generated symbols are shown with $\hat{}$ and $\bar{}$, respectively.
The receiver is not aware yet that which symbols are healthy and which ones are corrupted. 
It is assumed that the two combinations, \textit{i.e.,} $\hat{x}_1, \hat{x}_2, \hat{x}_3, \hat{x}_5, \hat{r}_1$ and $\hat{x}_1, \hat{x}_2, \hat{x}_5, \hat{r}_1, \hat{r}_2$ have generated the same CRC and hence the same encoded data.
Accordingly, $\hat{x}_2 = \bar{x}_2$ and $\hat{r}_2 = \bar{r}_2$. 
Thus, any combination out of the set $\hat{x}_1, \hat{x}_2, \hat{x}_3, \hat{x}_5, \hat{r}_1, \hat{r}_2$ generates the same encoded data. 
In total, ${6 \choose 5} = 6$ combinations exist which would generate the same CRC.
Note that in this example, $b = 1$.  

Accordingly, each CRC repeats ${k+i \choose k}$ where $i \ge 0$.  

\subsection{A Successful Data Retrieval}

\begin{figure}[t]
\center
\includegraphics[width=0.45\textwidth]{pic/crc.pdf}
\caption{An example of the pattern of the CRCs repetitions in case of a successful data retrieval.}
\label{success}
\end{figure} 

Fig.~\ref{success} shows an example of the number of CRCs repetitions for a successful data retrieval. 
It is assumed in this example that a minimum of $k+1$ symbols of the encoded data are healthy in addition to some of the bytes from the CRC (but not all the bytes).
This is similar to Example.~\ref{ex:scheme}.~(b).
In this case, at least one CRC will be repeated ${k+1 \choose k}=k+1$~times. 
As soon as the receiver finds one CRC with $k+1$ repetitions and a minimum of $2$ common bytes with the CRC, it stops the process as data can be retrieved.
At this time, Normally, there are a lot of CRCs which are repeated only once such as CRC\#1, CRC\#2 and CRC\#3 in Fig.~\ref{success}. 
There could be a few CRCs which are repeated more than once apart from the one which is repeated $k+1$~times. 

On the other hand, let us consider a healthy CRC and a minimum of $k$ healthy symbols such as Fig.~\ref{idea}.~(a).
In such a case, data can be retrieved as soon as the correct symbols are selected. 
The correct symbols might be the first choice or even the last choice.
Thus, the number of CRCs repetitions depends on the time of selecting the healthy symbols.

\subsection{A Failed Data Retrieval}

Assuming using brute force for trying different combinations, a failed data retrieval means that the receiver has tried all the different combinations.
Fig.~\ref{fail} shows an example for the number of CRCs repetitions for a failed data retrieval. 
CRC\#1 which is repeated only twice shows a collision in CRC calculation where two different encoded datas are mapped to the same CRC.
Every other CRC is repeated either once or ${k+i \choose k}$ times.

\begin{figure}[t]
\center
\includegraphics[width=0.45\textwidth]{pic/crcfail.pdf}
\caption{An example of the pattern of the CRCs repetitions in case of a failed data retrieval.}
\label{fail}
\end{figure} 

  

